Spectal Harmonics: Bridging Spectral Embedding and Matrix Completion in Self-Supervised Learning

Self-supervised methods received tremendous attention thanks to their seemingly heuristic approach to learning representations that respect the semantics of the data without any apparent supervision in the form of labels. A growing body of literature is already being published in an attempt to build a coherent and theoretically grounded understanding of the workings of a zoo of losses used in modern self-supervised representation learning methods. In this paper, we attempt to provide an understanding from the perspective of a Laplace operator and connect the inductive bias stemming from the augmentation process to a low-rank matrix completion problem. To this end, we leverage the results from low-rank matrix completion to provide theoretical analysis on the convergence of modern SSL methods and a key property that affects their downstream performance.

==> figures/data/coh-layers.tex <==
coh l
10	2
5	3

==> figures/data/mu-len.tex <==
mu	 len	std
8.089658260345459	1	0.5801310964192642
10.3669864654541		2	1.4868258985457479
11.959936237335205	3	0.992042888624425	
14.545428911844889	4	2.4969116371613533

==> figures/data/mu-param.tex <==
p	 mu
0.525312	7.26
1.050624	9.49
1.574912	10.47
5.246976	
2.901172	12.47
9.443328	

==> figures/data/p-opt.tex <==
epoch	p	q
1	0.006531748381458499	2e-05
2	0.0034624994094241165	2e-05
3	0.00238501185937114	2e-05
4	0.0018295623140594916	2e-05
5	0.0014889695240720932	2e-05
6	0.0012580476692505256	2e-05
7	0.0010908202760665532	2e-05
8	0.0009639374617034626	2e-05
9	0.0008642580860853713	2e-05
10	0.0007838098057750198	2e-05
11	0.0007174701253279537	2e-05
12	0.0006617947044077405	2e-05
13	0.0006143806091655251	2e-05
14	0.0005734994549896862	2e-05
15	0.0005378756544676925	2e-05
16	0.0005065468831885896	2e-05
17	0.00047877323127026346	2e-05
18	0.00045397628956433744	2e-05
19	0.00043169724916421436	2e-05
20	0.00041156742475699666	2e-05
21	0.0003932871013867045	2e-05
22	0.00037661008254532836	2e-05
23	0.0003613322217059773	2e-05
24	0.00034728278709510917	2e-05
25	0.0003343178743704973	2e-05
26	0.0003223153214054446	2e-05
27	0.00031117073968234304	2e-05
28	0.0003007943859730479	2e-05
29	0.000291108673538739	2e-05
30	0.00028204617514683734	2e-05
31	0.0002735480079817014	2e-05
32	0.00026556251776272403	2e-05
33	0.0002580441992503761	2e-05
34	0.0002509528049701239	2e-05
35	0.00024425260489622396	2e-05
36	0.00023791176804299465	2e-05
37	0.00023190184313658118	2e-05
38	0.0002261973203028896	2e-05
39	0.00022077525937966018	2e-05
40	0.00021561497331324168	2e-05
41	0.00021069775733201964	2e-05
42	0.00020600665634548876	2e-05
43	0.00020152626441017664	2e-05
44	0.00019724255121333993	2e-05
45	0.0001931427114148957	2e-05
46	0.0001892150334049394	2e-05
47	0.0001854487846149121	2e-05
48	0.00018183411099317406	2e-05
49	0.0001783619486423112	2e-05
50	0.00017502394593304333	2e-05
51	0.00017181239467155686	2e-05
52	0.00016872016911406335	2e-05
53	0.00016574067180281284	2e-05
54	0.0001628677853483888	2e-05
55	0.00016009582940926283	2e-05
56	0.00015741952222562633	2e-05
57	0.0001548339461539473	2e-05
58	0.00015233451672436488	2e-05
59	0.00014991695480724948	2e-05
60	0.0001475772615299142	2e-05
61	0.00014531169563112672	2e-05
62	0.00014311675298100767	2e-05
63	0.00014098914802818593	2e-05
64	0.0001389257969655766	2e-05
65	0.0001369238024315968	2e-05
66	0.00013498043958563857	2e-05
67	0.00013309314341568886	2e-05
68	0.00013125949715255802	2e-05
69	0.0001294772216796	2e-05
70	0.00012774416583939392	2e-05
71	0.00012605829754985874	2e-05
72	0.0001244176956519103	2e-05
73	0.00012282054241922989	2e-05
74	0.00012126511666815188	2e-05
75	0.00011974978741223137	2e-05
76	0.00011827300801183607	2e-05
77	0.00011683331077421903	2e-05
78	0.00011542930196405745	2e-05
79	0.0001140596571884573	2e-05
80	0.0001127231171239925	2e-05
81	0.00011141848355652078	2e-05
82	0.00011014461570734804	2e-05
83	0.00010890042682183707	2e-05
84	0.00010768488099881263	2e-05
85	0.00010649699024113466	2e-05
86	0.0001053358117096201	2e-05
87	0.000104200445164119	2e-05
88	0.00010309003057700788	2e-05
89	0.00010200374590567816	2e-05
90	0.00010094080501177822	2e-05
91	9.990045571603517e-05	2e-05
92	9.888197797844507e-05	2e-05
93	9.7884682194491e-05	2e-05
94	9.690790759883621e-05	2e-05
95	9.595102076865302e-05	2e-05
96	9.501341421939676e-05	2e-05
97	9.409450508641967e-05	2e-05
98	9.319373388635696e-05	2e-05
99	9.231056335270032e-05	2e-05
100	9.1444477340419e-05	2e-05
101	9.0594979794891e-05	2e-05
102	8.976159378077583e-05	2e-05
103	8.894386056679596e-05	2e-05
104	8.81413387627022e-05	2e-05
105	8.735360350497867e-05	2e-05
106	8.658024568810203e-05	2e-05
107	8.582087123840374e-05	2e-05
108	8.507510042780303e-05	2e-05
109	8.434256722487491e-05	2e-05
110	8.362291868090173e-05	2e-05
111	8.291581434872455e-05	2e-05
112	8.222092573236436e-05	2e-05
113	8.153793576552682e-05	2e-05
114	8.086653831723445e-05	2e-05
115	8.02064377229517e-05	2e-05
116	7.955734833968015e-05	2e-05
117	7.8918994123604e-05	2e-05
118	7.829110822896146e-05	2e-05
119	7.767343262690632e-05	2e-05
120	7.706571774320491e-05	2e-05
121	7.646772211368993e-05	2e-05
122	7.587921205646281e-05	2e-05
123	7.529996135990021e-05	2e-05
124	7.472975098558235e-05	2e-05
125	7.416836878531519e-05	2e-05
126	7.361560923147182e-05	2e-05
127	7.307127315992589e-05	2e-05
128	7.253516752489558e-05	2e-05
129	7.200710516505827e-05	2e-05
130	7.148690458033482e-05	2e-05
131	7.09743897187795e-05	2e-05
132	7.046938977304453e-05	2e-05
133	6.997173898592065e-05	2e-05
134	6.948127646448423e-05	2e-05
135	6.89978460024091e-05	2e-05
136	6.852129591002706e-05	2e-05
137	6.805147885174518e-05	2e-05
138	6.758825169045024e-05	2e-05
139	6.713147533855222e-05	2e-05
140	6.66810146153379e-05	2e-05
141	6.623673811032475e-05	2e-05
142	6.579851805232186e-05	2e-05
143	6.53662301839218e-05	2e-05
144	6.493975364116164e-05	2e-05
145	6.451897083810619e-05	2e-05
146	6.410376735611995e-05	2e-05
147	6.36940318376066e-05	2e-05
148	6.328965588400657e-05	2e-05
149	6.289053395785531e-05	2e-05
150	6.24965632887139e-05	2e-05
151	6.210764378279474e-05	2e-05
152	6.172367793611362e-05	2e-05
153	6.134457075100863e-05	2e-05
154	6.097022965587402e-05	2e-05
155	6.060056442796586e-05	2e-05
156	6.0235487119142395e-05	2e-05
157	5.987491198440994e-05	2e-05
158	5.951875541315103e-05	2e-05
159	5.916693586291824e-05	2e-05
160	5.8819373795682084e-05	2e-05
161	5.847599161642767e-05	2e-05
162	5.813671361399949e-05	2e-05
163	5.7801465904098895e-05	2e-05
164	5.747017637434312e-05	2e-05
165	5.7142774631299266e-05	2e-05
166	5.681919194941091e-05	2e-05
167	5.649936122173876e-05	2e-05
168	5.618321691244045e-05	2e-05
169	5.587069501091808e-05	2e-05
170	5.556173298756576e-05	2e-05
171	5.5256269751052124e-05	2e-05
172	5.495424560707596e-05	2e-05
173	5.465560221853584e-05	2e-05
174	5.436028256705795e-05	2e-05
175	5.4068230915827466e-05	2e-05
176	5.3779392773672874e-05	2e-05
177	5.34937148603539e-05	2e-05
178	5.3211145073006115e-05	2e-05
179	5.293163245369752e-05	2e-05
180	5.2655127158054306e-05	2e-05
181	5.238158042491472e-05	2e-05
182	5.211094454697217e-05	2e-05
183	5.184317284236967e-05	2e-05
184	5.157821962721022e-05	2e-05
185	5.1316040188948484e-05	2e-05
186	5.105659076063117e-05	2e-05
187	5.079982849595439e-05	2e-05
188	5.0545711445108166e-05	2e-05
189	5.029419853137903e-05	2e-05
190	5.004524952848301e-05	2e-05
191	4.97988250386028e-05	2e-05
192	4.9554886471103236e-05	2e-05
193	4.931339602190121e-05	2e-05
194	4.907431665346619e-05	2e-05
195	4.8837612075429295e-05	2e-05
196	4.860324672577916e-05	2e-05
197	4.837118575262404e-05	2e-05
198	4.814139499650034e-05	2e-05
199	4.791384097320853e-05	2e-05
200	4.7688490857158164e-05	2e-05
201	4.7465312465204346e-05	2e-05
202	4.724427424095903e-05	2e-05
203	4.702534523956062e-05	2e-05
204	4.68084951128866e-05	2e-05
205	4.6593694095194006e-05	2e-05
206	4.638091298917339e-05	2e-05
207	4.6170123152402515e-05	2e-05
208	4.5961296484186346e-05	2e-05
209	4.575440541277064e-05	2e-05
210	4.554942288291663e-05	2e-05
211	4.5346322343825205e-05	2e-05
212	4.51450777373988e-05	2e-05
213	4.494566348683047e-05	2e-05
214	4.474805448550904e-05	2e-05
215	4.4552226086230523e-05	2e-05
216	4.4358154090705844e-05	2e-05
217	4.416581473935538e-05	2e-05
218	4.397518470138118e-05	2e-05
219	4.378624106510823e-05	2e-05
220	4.359896132858602e-05	2e-05
221	4.3413323390442564e-05	2e-05
222	4.3229305540982694e-05	2e-05
223	4.304688645352327e-05	2e-05
224	4.286604517595778e-05	2e-05
225	4.268676112254344e-05	2e-05
226	4.250901406590383e-05	2e-05
227	4.233278412924057e-05	2e-05
228	4.215805177874764e-05	2e-05
229	4.198479781622219e-05	2e-05
230	4.181300337186599e-05	2e-05
231	4.16426498972718e-05	2e-05
232	4.1473719158588936e-05	2e-05
233	4.1306193229863e-05	2e-05
234	4.114005448654445e-05	2e-05
235	4.097528559916099e-05	2e-05
236	4.08118695271491e-05	2e-05
237	4.064978951283987e-05	2e-05
238	4.048902907559491e-05	2e-05
239	4.032957200608769e-05	2e-05
240	4.017140236072633e-05	2e-05
241	4.001450445621366e-05	2e-05
242	3.9858862864240565e-05	2e-05
243	3.970446240630907e-05	2e-05
244	3.955128814868113e-05	2e-05
245	3.9399325397449864e-05	2e-05
246	3.924855969372951e-05	2e-05
247	3.9098976808961134e-05	2e-05
248	3.895056274033042e-05	2e-05
249	3.8803303706294774e-05	2e-05
250	3.8657186142216535e-05	2e-05
251	3.851219669609942e-05	2e-05
252	3.836832222442533e-05	2e-05
253	3.8225549788088815e-05	2e-05
254	3.808386664842646e-05	2e-05
255	3.794326026333869e-05	2e-05
256	3.780371828350144e-05	2e-05
257	3.76652285486653e-05	2e-05
258	3.752777908403973e-05	2e-05
259	3.739135809676015e-05	2e-05
260	3.725595397243562e-05	2e-05
261	3.712155527177499e-05	2e-05
262	3.69881507272895e-05	2e-05
263	3.685572924006971e-05	2e-05
264	3.67242798766349e-05	2e-05
265	3.659379186585301e-05	2e-05
266	3.6464254595929254e-05	2e-05
267	3.6335657611461715e-05	2e-05
268	3.6207990610562025e-05	2e-05
269	3.608124344203965e-05	2e-05
270	3.595540610264801e-05	2e-05
271	3.583046873439087e-05	2e-05
272	3.570642162188755e-05	2e-05
273	3.558325518979532e-05	2e-05
274	3.5460960000287675e-05	2e-05
275	3.5339526750587e-05	2e-05
276	3.5218946270550247e-05	2e-05
277	3.509920952030638e-05	2e-05
278	3.498030758794422e-05	2e-05
279	3.486223168724941e-05	2e-05
280	3.474497315548944e-05	2e-05
281	3.462852345124534e-05	2e-05
282	3.451287415228909e-05	2e-05
283	3.439801695350543e-05	2e-05
284	3.4283943664857183e-05	2e-05
285	3.417064620939284e-05	2e-05
286	3.405811662129564e-05	2e-05
287	3.394634704397275e-05	2e-05
288	3.383532972818406e-05	2e-05
289	3.37250570302092e-05	2e-05
290	3.3615521410052174e-05	2e-05
291	3.350671542968257e-05	2e-05
292	3.33986317513125e-05	2e-05
293	3.3291263135708423e-05	2e-05
294	3.318460244053708e-05	2e-05
295	3.30786426187447e-05	2e-05
296	3.2973376716968605e-05	2e-05
297	3.286879787398065e-05	2e-05
298	3.276489931916166e-05	2e-05
299	3.266167437100604e-05	2e-05
300	3.2559116435656064e-05	2e-05
301	3.245721900546501e-05	2e-05
302	3.235597565758855e-05	2e-05
303	3.225538005260367e-05	2e-05
304	3.215542593315463e-05	2e-05
305	3.205610712262523e-05	2e-05
306	3.195741752383677e-05	2e-05
307	3.185935111777129e-05	2e-05
308	3.176190196231926e-05	2e-05
309	3.166506419105147e-05	2e-05
310	3.156883201201433e-05	2e-05
311	3.147319970654817e-05	2e-05
312	3.137816162812804e-05	2e-05
313	3.128371220122647e-05	2e-05
314	3.118984592019774e-05	2e-05
315	3.109655734818311e-05	2e-05
316	3.100384111603669e-05	2e-05
317	3.091169192127135e-05	2e-05
318	3.0820104527024324e-05	2e-05
319	3.072907376104208e-05	2e-05
320	3.063859451468396e-05	2e-05
321	3.054866174194431e-05	2e-05
322	3.0459270458492503e-05	2e-05
323	3.037041574073081e-05	2e-05
324	3.0282092724869286e-05	2e-05
325	3.0194296606017717e-05	2e-05
326	3.0107022637294035e-05	2e-05
327	3.0020266128948886e-05	2e-05
328	2.993402244750612e-05	2e-05
329	2.9848287014918674e-05	2e-05
330	2.9763055307739735e-05	2e-05
331	2.967832285630868e-05	2e-05
332	2.959408524395164e-05	2e-05
333	2.9510338106196225e-05	2e-05
334	2.942707713000032e-05	2e-05
335	2.934429805299439e-05	2e-05
336	2.9261996662737288e-05	2e-05
337	2.9180168795985146e-05	2e-05
338	2.9098810337973035e-05	2e-05
339	2.90179172217093e-05	2e-05
340	2.8937485427282102e-05	2e-05
341	2.8857510981178107e-05	2e-05
342	2.8777989955613008e-05	2e-05
343	2.8698918467873542e-05	2e-05
344	2.862029267967092e-05	2e-05
345	2.854210879650541e-05	2e-05
346	2.846436306704172e-05	2e-05
347	2.8387051782495166e-05	2e-05
348	2.8310171276028213e-05	2e-05
349	2.823371792215738e-05	2e-05
350	2.8157688136170118e-05	2e-05
351	2.8082078373551538e-05	2e-05
352	2.8006885129420905e-05	2e-05
353	2.793210493797752e-05	2e-05
354	2.7857734371955863e-05	2e-05
355	2.7783770042089963e-05	2e-05
356	2.7710208596586582e-05	2e-05
357	2.763704672060721e-05	2e-05
358	2.7564281135758634e-05	2e-05
359	2.7491908599591942e-05	2e-05
360	2.7419925905109737e-05	2e-05
361	2.734832988028157e-05	2e-05
362	2.7277117387567128e-05	2e-05
363	2.7206285323447394e-05	2e-05
364	2.7135830617963374e-05	2e-05
365	2.706575023426232e-05	2e-05
366	2.699604116815132e-05	2e-05
367	2.6926700447658103e-05	2e-05
368	2.6857725132598946e-05	2e-05
369	2.6789112314153512e-05	2e-05
370	2.6720859114446492e-05	2e-05
371	2.6652962686135996e-05	2e-05
372	2.6585420212008416e-05	2e-05
373	2.6518228904579854e-05	2e-05
374	2.6451386005703758e-05	2e-05
375	2.638488878618485e-05	2e-05
376	2.6318734545399127e-05	2e-05
377	2.6252920610919784e-05	2e-05
378	2.6187444338149125e-05	2e-05
379	2.6122303109956136e-05	2e-05
380	2.6057494336319754e-05	2e-05
381	2.5993015453977714e-05	2e-05
382	2.5928863926080807e-05	2e-05
383	2.5865037241852547e-05	2e-05
384	2.580153291625405e-05	2e-05
385	2.5738348489654112e-05	2e-05
386	2.567548152750432e-05	2e-05
387	2.5612929620019216e-05	2e-05
388	2.5550690381861276e-05	2e-05
389	2.5488761451830734e-05	2e-05
390	2.5427140492560123e-05	2e-05
391	2.5365825190213448e-05	2e-05
392	2.5304813254189923e-05	2e-05
393	2.5244102416832154e-05	2e-05
394	2.518369043313875e-05	2e-05
395	2.5123575080481248e-05	2e-05
396	2.5063754158325247e-05	2e-05
397	2.500422548795576e-05	2e-05
398	2.494498691220661e-05	2e-05
399	2.4886036295193903e-05	2e-05
400	2.4827371522053422e-05	2e-05
401	2.476899049868188e-05	2e-05
402	2.4710891151482108e-05	2e-05
403	2.4653071427111837e-05	2e-05
404	2.4595529292236282e-05	2e-05
405	2.4538262733284315e-05	2e-05
406	2.4481269756208224e-05	2e-05
407	2.4424548386246917e-05	2e-05
408	2.4368096667692647e-05	2e-05
409	2.431191266366107e-05	2e-05
410	2.4255994455864648e-05	2e-05
411	2.4200340144389314e-05	2e-05
412	2.41449478474744e-05	2e-05
413	2.4089815701295628e-05	2e-05
414	2.4034941859751338e-05	2e-05
415	2.3980324494251667e-05	2e-05
416	2.3925961793510807e-05	2e-05
417	2.3871851963342155e-05	2e-05
418	2.3817993226456456e-05	2e-05
419	2.376438382226271e-05	2e-05
420	2.371102200667197e-05	2e-05
421	2.365790605190387e-05	2e-05
422	2.3605034246295858e-05	2e-05
423	2.3552404894115154e-05	2e-05
424	2.35000163153733e-05	2e-05
425	2.344786684564332e-05	2e-05
426	2.3395954835879402e-05	2e-05
427	2.3344278652239116e-05	2e-05
428	2.3292836675908097e-05	2e-05
429	2.3241627302927132e-05	2e-05
430	2.3190648944021614e-05	2e-05
431	2.313990002443344e-05	2e-05
432	2.3089378983755082e-05	2e-05
433	2.3039084275766057e-05	2e-05
434	2.298901436827155e-05	2e-05
435	2.293916774294326e-05	2e-05
436	2.288954289516246e-05	2e-05
437	2.2840138333865106e-05	2e-05
438	2.2790952581389125e-05	2e-05
439	2.274198417332368e-05	2e-05
440	2.269323165836059e-05	2e-05
441	2.2644693598147594e-05	2e-05
442	2.2596368567143753e-05	2e-05
443	2.2548255152476646e-05	2e-05
444	2.250035195380156e-05	2e-05
445	2.2452657583162518e-05	2e-05
446	2.2405170664855203e-05	2e-05
447	2.2357889835291635e-05	2e-05
448	2.2310813742866687e-05	2e-05
449	2.2263941047826364e-05	2e-05
450	2.2217270422137795e-05	2e-05
451	2.2170800549360973e-05	2e-05
452	2.2124530124522117e-05	2e-05
453	2.2078457853988803e-05	2e-05
454	2.2032582455346576e-05	2e-05
455	2.198690265727729e-05	2e-05
456	2.1941417199439023e-05	2e-05
457	2.1896124832347474e-05	2e-05
458	2.1851024317258983e-05	2e-05
459	2.1806114426054994e-05	2e-05
460	2.176139394112807e-05	2e-05
461	2.1716861655269342e-05	2e-05
462	2.1672516371557406e-05	2e-05
463	2.1628356903248617e-05	2e-05
464	2.1584382073668892e-05	2e-05
465	2.1540590716106734e-05	2e-05
466	2.1496981673707755e-05	2e-05
467	2.145355379937047e-05	2e-05
468	2.1410305955643453e-05	2e-05
469	2.1367237014623728e-05	2e-05
470	2.132434585785653e-05	2e-05
471	2.128163137623626e-05	2e-05
472	2.1239092469908732e-05	2e-05
473	2.1196728048174602e-05	2e-05
474	2.1154537029394056e-05	2e-05
475	2.1112518340892642e-05	2e-05
476	2.1070670918868317e-05	2e-05
477	2.1028993708299625e-05	2e-05
478	2.0987485662855002e-05	2e-05
479	2.0946145744803263e-05	2e-05
480	2.0904972924925115e-05	2e-05
481	2.086396618242584e-05	2e-05
482	2.0823124504849014e-05	2e-05
483	2.0782446887991254e-05	2e-05
484	2.0741932335818077e-05	2e-05
485	2.070157986038077e-05	2e-05
486	2.0661388481734233e-05	2e-05
487	2.0621357227855862e-05	2e-05
488	2.058148513456543e-05	2e-05
489	2.054177124544589e-05	2e-05
490	2.05022146117652e-05	2e-05
491	2.046281429239903e-05	2e-05
492	2.0423569353754458e-05	2e-05
493	2.038447886969455e-05	2e-05
494	2.0345541921463835e-05	2e-05
495	2.030675759761474e-05	2e-05
496	2.0268124993934836e-05	2e-05
497	2.0229643213374936e-05	2e-05
498	2.0191311365978177e-05	2e-05
499	2.0153128568809768e-05	2e-05
500	2.011509394588773e-05	2e-05
501	2.007720662811436e-05	2e-05
502	2.0039465753208542e-05	2e-05
503	2.0001870465638826e-05	2e-05
504	1.9964419916557374e-05	2e-05
505	1.9927113263734567e-05	2e-05
506	1.988994967149447e-05	2e-05
507	1.9852928310651035e-05	2e-05
508	1.981604835844499e-05	2e-05
509	1.9779308998481555e-05	2e-05
510	1.974270942066882e-05	2e-05
511	1.970624882115686e-05	2e-05
512	1.9669926402277547e-05	2e-05
513	1.963374137248506e-05	2e-05
514	1.959769294629711e-05	2e-05
515	1.95617803442368e-05	2e-05
516	1.9526002792775162e-05	2e-05
517	1.9490359524274394e-05	2e-05
518	1.9454849776931684e-05	2e-05
519	1.9419472794723743e-05	2e-05
520	1.938422782735191e-05	2e-05
521	1.9349114130187933e-05	2e-05
522	1.9314130964220315e-05	2e-05
523	1.9279277596001344e-05	2e-05
524	1.9244553297594625e-05	2e-05
525	1.920995734652329e-05	2e-05
526	1.917548902571876e-05	2e-05
527	1.914114762347006e-05	2e-05
528	1.910693243337376e-05	2e-05
529	1.9072842754284418e-05	2e-05
530	1.903887789026562e-05	2e-05
531	1.900503715054155e-05	2e-05
532	1.8971319849449086e-05	2e-05
533	1.8937725306390494e-05	2e-05
534	1.8904252845786538e-05	2e-05
535	1.887090179703022e-05	2e-05
536	1.883767149444096e-05	2e-05
537	1.8804561277219324e-05	2e-05
538	1.877157048940223e-05	2e-05
539	1.8738698479818627e-05	2e-05
540	1.8705944602045734e-05	2e-05
541	1.8673308214365663e-05	2e-05
542	1.8640788679722615e-05	2e-05
543	1.8608385365680456e-05	2e-05
544	1.8576097644380784e-05	2e-05
545	1.8543924892501523e-05	2e-05
546	1.8511866491215855e-05	2e-05
547	1.8479921826151654e-05	2e-05
548	1.844809028735138e-05	2e-05
549	1.841637126923237e-05	2e-05
550	1.838476417054756e-05	2e-05
551	1.835326839434665e-05	2e-05
552	1.8321883347937684e-05	2e-05
553	1.829060844284901e-05	2e-05
554	1.82594430947917e-05	2e-05
555	1.822838672362233e-05	2e-05
556	1.819743875330616e-05	2e-05
557	1.816659861188076e-05	2e-05
558	1.8135865731419924e-05	2e-05
559	1.8105239547998073e-05	2e-05
560	1.8074719501654955e-05	2e-05
561	1.804430503636077e-05	2e-05
562	1.801399559998163e-05	2e-05
563	1.7983790644245397e-05	2e-05
564	1.7953689624707904e-05	2e-05
565	1.7923692000719467e-05	2e-05
566	1.789379723539182e-05	2e-05
567	1.7864004795565356e-05	2e-05
568	1.7834314151776708e-05	2e-05
569	1.78047247782267e-05	2e-05
570	1.7775236152748583e-05	2e-05
571	1.774584775677666e-05	2e-05
572	1.771655907531518e-05	2e-05
573	1.7687369596907602e-05	2e-05
574	1.765827881360612e-05	2e-05
575	1.7629286220941588e-05	2e-05
576	1.760039131789365e-05	2e-05
577	1.7571593606861282e-05	2e-05
578	1.7542892593633547e-05	2e-05
579	1.7514287787360717e-05	2e-05
580	1.7485778700525627e-05	2e-05
581	1.7457364848915405e-05	2e-05
582	1.7429045751593407e-05	2e-05
583	1.7400820930871478e-05	2e-05
584	1.73726899122825e-05	2e-05
585	1.734465222455322e-05	2e-05
586	1.7316707399577302e-05	2e-05
587	1.7288854972388735e-05	2e-05
588	1.7261094481135436e-05	2e-05
589	1.723342546705317e-05	2e-05
590	1.7205847474439694e-05	2e-05
591	1.7178360050629198e-05	2e-05
592	1.7150962745966956e-05	2e-05
593	1.7123655113784287e-05	2e-05
594	1.7096436710373715e-05	2e-05
595	1.70693070949644e-05	2e-05
596	1.7042265829697834e-05	2e-05
597	1.7015312479603718e-05	2e-05
598	1.6988446612576153e-05	2e-05
599	1.6961667799350017e-05	2e-05
600	1.693497561347759e-05	2e-05
601	1.6908369631305403e-05	2e-05
602	1.6881849431951335e-05	2e-05
603	1.6855414597281915e-05	2e-05
604	1.682906471188986e-05	2e-05
605	1.6802799363071815e-05	2e-05
606	1.6776618140806346e-05	2e-05
607	1.6750520637732095e-05	2e-05
608	1.672450644912622e-05	2e-05
609	1.6698575172882966e-05	2e-05
610	1.6672726409492506e-05	2e-05
611	1.664695976201996e-05	2e-05
612	1.662127483608462e-05	2e-05
613	1.659567123983938e-05	2e-05
614	1.657014858395036e-05	2e-05
615	1.6544706481576734e-05	2e-05
616	1.6519344548350756e-05	2e-05
617	1.6494062402357958e-05	2e-05
618	1.646885966411754e-05	2e-05
619	1.6443735956563e-05	2e-05
620	1.6418690905022864e-05	2e-05
621	1.6393724137201673e-05	2e-05
622	1.6368835283161116e-05	2e-05
623	1.634402397530133e-05	2e-05
624	1.6319289848342438e-05	2e-05
625	1.629463253930618e-05	2e-05
626	1.6270051687497796e-05	2e-05
627	1.6245546934488013e-05	2e-05
628	1.6221117924095262e-05	2e-05
629	1.6196764302368016e-05	2e-05
630	1.6172485717567326e-05	2e-05
631	1.6148281820149494e-05	2e-05
632	1.612415226274894e-05	2e-05
633	1.61000967001612e-05	2e-05
634	1.6076114789326105e-05	2e-05
635	1.6052206189311106e-05	2e-05
636	1.6028370561294756e-05	2e-05
637	1.6004607568550352e-05	2e-05
638	1.598091687642971e-05	2e-05
639	1.5957298152347124e-05	2e-05
640	1.5933751065763437e-05	2e-05
641	1.5910275288170306e-05	2e-05
642	1.588687049307454e-05	2e-05
643	1.5863536355982672e-05	2e-05
644	1.5840272554385593e-05	2e-05
645	1.5817078767743384e-05	2e-05
646	1.579395467747026e-05	2e-05
647	1.5770899966919645e-05	2e-05
648	1.574791432136942e-05	2e-05
649	1.572499742800726e-05	2e-05
650	1.570214897591614e-05	2e-05
651	1.5679368656059967e-05	2e-05
652	1.5656656161269308e-05	2e-05
653	1.5634011186227305e-05	2e-05
654	1.5611433427455686e-05	2e-05
655	1.5588922583300887e-05	2e-05
656	1.5566478353920334e-05	2e-05
657	1.5544100441268833e-05	2e-05
658	1.552178854908507e-05	2e-05
659	1.5499542382878267e-05	2e-05
660	1.547736164991492e-05	2e-05
661	1.5455246059205668e-05	2e-05
662	1.5433195321492307e-05	2e-05
663	1.541120914923488e-05	2e-05
664	1.538928725659891e-05	2e-05
665	1.536742935944273e-05	2e-05
666	1.5345635175304924e-05	2e-05
667	1.5323904423391917e-05	2e-05
668	1.530223682456563e-05	2e-05
669	1.5280632101331258e-05	2e-05
670	1.5259089977825152e-05	2e-05
671	1.523761017980286e-05	2e-05
672	1.5216192434627176e-05	2e-05
673	1.519483647125638e-05	2e-05
674	1.5173542020232533e-05	2e-05
675	1.5152308813669918e-05	2e-05
676	1.5131136585243524e-05	2e-05
677	1.5110025070177682e-05	2e-05
678	1.508897400523479e-05	2e-05
679	1.5067983128704099e-05	2e-05
680	1.5047052180390654e-05	2e-05
681	1.5026180901604306e-05	2e-05
682	1.500536903514878e-05	2e-05
683	1.4984616325310926e-05	2e-05
684	1.4963922517849973e-05	2e-05
685	1.494328735998694e-05	2e-05
686	1.4922710600394105e-05	2e-05
687	1.4902191989184574e-05	2e-05
688	1.488173127790193e-05	2e-05
689	1.4861328219510026e-05	2e-05
690	1.4840982568382751e-05	2e-05
691	1.4820694080294025e-05	2e-05
692	1.4800462512407758e-05	2e-05
693	1.4780287623267977e-05	2e-05
694	1.4760169172788983e-05	2e-05
695	1.4740106922245647e-05	2e-05
696	1.4720100634263724e-05	2e-05
697	1.4700150072810305e-05	2e-05
698	1.4680255003184328e-05	2e-05
699	1.4660415192007154e-05	2e-05
700	1.4640630407213245e-05	2e-05
701	1.4620900418040942e-05	2e-05
702	1.4601224995023251e-05	2e-05
703	1.4581603909978774e-05	2e-05
704	1.4562036936002687e-05	2e-05
705	1.4542523847457808e-05	2e-05
706	1.4523064419965716e-05	2e-05
707	1.4503658430397969e-05	2e-05
708	1.4484305656867383e-05	2e-05
709	1.4465005878719398e-05	2e-05
710	1.4445758876523478e-05	2e-05
711	1.4426564432064656e-05	2e-05
712	1.4407422328335052e-05	2e-05
713	1.4388332349525559e-05	2e-05
714	1.4369294281017517e-05	2e-05
715	1.4350307909374524e-05	2e-05
716	1.433137302233425e-05	2e-05
717	1.4312489408800388e-05	2e-05
718	1.4293656858834598e-05	2e-05
719	1.4274875163648576e-05	2e-05
720	1.425614411559617e-05	2e-05
721	1.4237463508165546e-05	2e-05
722	1.421883313597144e-05	2e-05
723	1.4200252794747459e-05	2e-05
724	1.4181722281338441e-05	2e-05
725	1.4163241393692915e-05	2e-05
726	1.4144809930855562e-05	2e-05
727	1.4126427692959783e-05	2e-05
728	1.4108094481220332e-05	2e-05
729	1.408981009792596e-05	2e-05
730	1.4071574346432167e-05	2e-05
731	1.4053387031154002e-05	2e-05
732	1.4035247957558903e-05	2e-05
733	1.401715693215962e-05	2e-05
734	1.3999113762507165e-05	2e-05
735	1.3981118257183858e-05	2e-05
736	1.3963170225796395e-05	2e-05
737	1.3945269478968988e-05	2e-05
738	1.392741582833656e-05	2e-05
739	1.3909609086537978e-05	2e-05
740	1.3891849067209375e-05	2e-05
741	1.3874135584977493e-05	2e-05
742	1.3856468455453083e-05	2e-05
743	1.3838847495224385e-05	2e-05
744	1.3821272521850625e-05	2e-05
745	1.380374335385558e-05	2e-05
746	1.3786259810721206e-05	2e-05
747	1.3768821712881282e-05	2e-05
748	1.3751428881715155e-05	2e-05
749	1.3734081139541488e-05	2e-05
750	1.371677830961207e-05	2e-05
751	1.3699520216105696e-05	2e-05
752	1.3682306684122078e-05	2e-05
753	1.3665137539675796e-05	2e-05
754	1.3648012609690307e-05	2e-05
755	1.3630931721992017e-05	2e-05
756	1.3613894705304371e-05	2e-05
757	1.3596901389241991e-05	2e-05
758	1.3579951604304894e-05	2e-05
759	1.3563045181872716e-05	2e-05
760	1.3546181954199002e-05	2e-05
761	1.3529361754405528e-05	2e-05
762	1.3512584416476694e-05	2e-05
763	1.3495849775253914e-05	2e-05
764	1.3479157666430106e-05	2e-05
765	1.3462507926544165e-05	2e-05
766	1.3445900392975535e-05	2e-05
767	1.3429334903938786e-05	2e-05
768	1.3412811298478242e-05	2e-05
769	1.3396329416462666e-05	2e-05
770	1.3379889098579953e-05	2e-05
771	1.3363490186331908e-05	2e-05
772	1.3347132522029015e-05	2e-05
773	1.3330815948785291e-05	2e-05
774	1.331454031051314e-05	2e-05
775	1.3298305451918291e-05	2e-05
776	1.3282111218494727e-05	2e-05
777	1.3265957456519692e-05	2e-05
778	1.32498440130487e-05	2e-05
779	1.323377073591063e-05	2e-05
780	1.3217737473702795e-05	2e-05
781	1.3201744075786123e-05	2e-05
782	1.3185790392280297e-05	2e-05
783	1.3169876274058994e-05	2e-05
784	1.315400157274513e-05	2e-05
785	1.3138166140706148e-05	2e-05
786	1.3122369831049324e-05	2e-05
787	1.3106612497617159e-05	2e-05
788	1.3090893994982745e-05	2e-05
789	1.3075214178445188e-05	2e-05
790	1.30595729040251e-05	2e-05
791	1.3043970028460058e-05	2e-05
792	1.302840540920017e-05	2e-05
793	1.3012878904403602e-05	2e-05
794	1.2997390372932204e-05	2e-05
795	1.298193967434713e-05	2e-05
796	1.296652666890448e-05	2e-05
797	1.2951151217551027e-05	2e-05
798	1.2935813181919927e-05	2e-05
799	1.292051242432647e-05	2e-05
800	1.2905248807763876e-05	2e-05
801	1.2890022195899122e-05	2e-05
802	1.287483245306879e-05	2e-05
803	1.2859679444274933e-05	2e-05
804	1.2844563035181023e-05	2e-05
805	1.2829483092107852e-05	2e-05
806	1.2814439482029532e-05	2e-05
807	1.27994320725695e-05	2e-05
808	1.2784460731996522e-05	2e-05
809	1.2769525329220787e-05	2e-05
810	1.2754625733789978e-05	2e-05
811	1.2739761815885384e-05	2e-05
812	1.2724933446318071e-05	2e-05
813	1.2710140496525027e-05	2e-05
814	1.2695382838565392e-05	2e-05
815	1.2680660345116667e-05	2e-05
816	1.2665972889470997e-05	2e-05
817	1.2651320345531417e-05	2e-05
818	1.2636702587808208e-05	2e-05
819	1.262211949141519e-05	2e-05
820	1.2607570932066142e-05	2e-05
821	1.259305678607115e-05	2e-05
822	1.2578576930333021e-05	2e-05
823	1.2564131242343768e-05	2e-05
824	1.254971960018105e-05	2e-05
825	1.2535341882504662e-05	2e-05
826	1.2520997968553064e-05	2e-05
827	1.2506687738139926e-05	2e-05
828	1.2492411071650711e-05	2e-05
829	1.2478167850039231e-05	2e-05
830	1.2463957954824309e-05	2e-05
831	1.2449781268086387e-05	2e-05
832	1.2435637672464215e-05	2e-05
833	1.2421527051151535e-05	2e-05
834	1.240744928789378e-05	2e-05
835	1.2393404266984839e-05	2e-05
836	1.2379391873263793e-05	2e-05
837	1.2365411992111716e-05	2e-05
838	1.2351464509448461e-05	2e-05
839	1.2337549311729508e-05	2e-05
840	1.2323666285942813e-05	2e-05
841	1.2309815319605661e-05	2e-05
842	1.2295996300761592e-05	2e-05
843	1.2282209117977299e-05	2e-05
844	1.2268453660339556e-05	2e-05
845	1.2254729817452213e-05	2e-05
846	1.2241037479433148e-05	2e-05
847	1.2227376536911283e-05	2e-05
848	1.2213746881023602e-05	2e-05
849	1.22001484034122e-05	2e-05
850	1.2186580996221348e-05	2e-05
851	1.2173044552094575e-05	2e-05
852	1.2159538964171783e-05	2e-05
853	1.2146064126086359e-05	2e-05
854	1.2132619931962339e-05	2e-05
855	1.2119206276411556e-05	2e-05
856	1.2105823054530843e-05	2e-05
857	1.2092470161899222e-05	2e-05
858	1.2079147494575143e-05	2e-05
859	1.2065854949093717e-05	2e-05
860	1.2052592422463986e-05	2e-05
861	1.2039359812166201e-05	2e-05
862	1.2026157016149126e-05	2e-05
863	1.2012983932827346e-05	2e-05
864	1.1999840461078625e-05	2e-05
865	1.1986726500241234e-05	2e-05
866	1.1973641950111359e-05	2e-05
867	1.1960586710940462e-05	2e-05
868	1.19475606834327e-05	2e-05
869	1.1934563768742371e-05	2e-05
870	1.1921595868471325e-05	2e-05
871	1.1908656884666453e-05	2e-05
872	1.1895746719817162e-05	2e-05
873	1.1882865276852863e-05	2e-05
874	1.1870012459140487e-05	2e-05
875	1.1857188170482026e-05	2e-05
876	1.1844392315112067e-05	2e-05
877	1.183162479769536e-05	2e-05
878	1.1818885523324409e-05	2e-05
879	1.1806174397517047e-05	2e-05
880	1.179349132621408e-05	2e-05
881	1.1780836215776882e-05	2e-05
882	1.176820897298506e-05	2e-05
883	1.1755609505034116e-05	2e-05
884	1.1743037719533115e-05	2e-05
885	1.1730493524502379e-05	2e-05
886	1.1717976828371205e-05	2e-05
887	1.1705487539975572e-05	2e-05
888	1.1693025568555885e-05	2e-05
889	1.1680590823754738e-05	2e-05
890	1.1668183215614669e-05	2e-05
891	1.1655802654575954e-05	2e-05
892	1.164344905147439e-05	2e-05
893	1.163112231753913e-05	2e-05
894	1.1618822364390489e-05	2e-05
895	1.1606549104037793e-05	2e-05
896	1.1594302448877242e-05	2e-05
897	1.1582082311689772e-05	2e-05
898	1.1569888605638942e-05	2e-05
899	1.1557721244268825e-05	2e-05
900	1.1545580141501933e-05	2e-05
901	1.1533465211637136e-05	2e-05
902	1.1521376369347594e-05	2e-05
903	1.1509313529678725e-05	2e-05
904	1.1497276608046166e-05	2e-05
905	1.1485265520233736e-05	2e-05
906	1.1473280182391458e-05	2e-05
907	1.1461320511033547e-05	2e-05
908	1.144938642303643e-05	2e-05
909	1.1437477835636779e-05	2e-05
910	1.1425594666429561e-05	2e-05
911	1.1413736833366093e-05	2e-05
912	1.1401904254752116e-05	2e-05
913	1.1390096849245857e-05	2e-05
914	1.1378314535856162e-05	2e-05
915	1.1366557233940566e-05	2e-05
916	1.1354824863203434e-05	2e-05
917	1.1343117343694103e-05	2e-05
918	1.1331434595804982e-05	2e-05
919	1.1319776540269771e-05	2e-05
920	1.1308143098161571e-05	2e-05
921	1.1296534190891105e-05	2e-05
922	1.1284949740204883e-05	2e-05
923	1.1273389668183422e-05	2e-05
924	1.1261853897239452e-05	2e-05
925	1.1250342350116149e-05	2e-05
926	1.1238854949885362e-05	2e-05
927	1.1227391619945876e-05	2e-05
928	1.121595228402166e-05	2e-05
929	1.1204536866160141e-05	2e-05
930	1.11931452907305e-05	2e-05
931	1.1181777482421937e-05	2e-05
932	1.1170433366242e-05	2e-05
933	1.11591128675149e-05	2e-05
934	1.114781591187981e-05	2e-05
935	1.1136542425289236e-05	2e-05
936	1.1125292334007337e-05	2e-05
937	1.1114065564608298e-05	2e-05
938	1.1102862043974692e-05	2e-05
939	1.1091681699295855e-05	2e-05
940	1.1080524458066279e-05	2e-05
941	1.1069390248084011e-05	2e-05
942	1.1058278997449058e-05	2e-05
943	1.1047190634561808e-05	2e-05
944	1.1036125088121458e-05	2e-05
945	1.1025082287124446e-05	2e-05
946	1.1014062160862918e-05	2e-05
947	1.1003064638923162e-05	2e-05
948	1.0992089651184087e-05	2e-05
949	1.098113712781571e-05	2e-05
950	1.097020699927762e-05	2e-05
951	1.0959299196317495e-05	2e-05
952	1.0948413649969594e-05	2e-05
953	1.0937550291553282e-05	2e-05
954	1.0926709052671547e-05	2e-05
955	1.0915889865209529e-05	2e-05
956	1.090509266133308e-05	2e-05
957	1.0894317373487296e-05	2e-05
958	1.0883563934395088e-05	2e-05
959	1.0872832277055749e-05	2e-05
960	1.0862122334743529e-05	2e-05
961	1.085143404100623e-05	2e-05
962	1.084076732966379e-05	2e-05
963	1.0830122134806898e-05	2e-05
964	1.08194983907956e-05	2e-05
965	1.0808896032257927e-05	2e-05
966	1.0798314994088515e-05	2e-05
967	1.078775521144726e-05	2e-05
968	1.0777216619757937e-05	2e-05
969	1.0766699154706887e-05	2e-05
970	1.0756202752241657e-05	2e-05
971	1.0745727348569686e-05	2e-05
972	1.0735272880156966e-05	2e-05
973	1.0724839283726753e-05	2e-05
974	1.0714426496258255e-05	2e-05
975	1.0704034454985314e-05	2e-05
976	1.0693663097395148e-05	2e-05
977	1.0683312361227054e-05	2e-05
978	1.067298218447114e-05	2e-05
979	1.0662672505367055e-05	2e-05
980	1.0652383262402737e-05	2e-05
981	1.0642114394313155e-05	2e-05
982	1.0631865840079083e-05	2e-05
983	1.0621637538925837e-05	2e-05
984	1.061142943032208e-05	2e-05
985	1.060124145397858e-05	2e-05
986	1.0591073549847001e-05	2e-05
987	1.0580925658118707e-05	2e-05
988	1.0570797719223548e-05	2e-05
989	1.0560689673828693e-05	2e-05
990	1.0550601462837406e-05	2e-05
991	1.054053302738792e-05	2e-05
992	1.0530484308852227e-05	2e-05
993	1.0520455248834938e-05	2e-05
994	1.0510445789172111e-05	2e-05
995	1.0500455871930114e-05	2e-05
996	1.0490485439404484e-05	2e-05
997	1.0480534434118774e-05	2e-05
998	1.0470602798823454e-05	2e-05
999	1.046069047649476e-05	2e-05


==> figures/data/perf-coh-2.tex <==
acc	 mu	 label
85.05	24.312	 a
82.64	50.023	 b


==> figures/data/perf-coh-3.tex <==
acc	 mu	 label
85.36	22.485	 a
82.64	40.054	 b


==> figures/data/perf-coh-4.tex <==
acc	 mu	 label
85.27	20.329	 a
83.98	43.184	 b


==> figures/data/perf-coh-5.tex <==
acc	 mu	 label
84.69	24.801	 a
82.85	57.476	 b


==> figures/data/perf-coh-6.tex <==
acc	 mu	 label
85.84	31.174	 a
84.69	62.544	 b


==> figures/data/perf-coh-7.tex <==
acc	 mu	 label
85.28	10.772	 a
84.04	55.614	 b


==> figures/data/perf-coh-8.tex <==
acc	 mu	 label
85.43	22.271	 a
83.32	82.488	 b


==> figures/data/perf-coh-9-0.tex <==
mu	 acc	 label
22.872	84.540	a
95.987	77.250	b


==> figures/data/perf-coh-9-1.tex <==
mu	 acc	 label
7.884	87.750	a
39.886	81.900	b


==> figures/data/perf-coh-9-2.tex <==
mu	 acc	 label
11.821	85.930	a
95.957	77.980	b


==> figures/data/perf-coh-9-3.tex <==
mu	 acc	 label
8.795	86.250	a
16.787	84.940	b


==> figures/data/perf-coh-9-4.tex <==
mu	 acc	 label
8.601	85.620	a
16.807	83.990	b


==> figures/data/perf-coh-9-5.tex <==
mu	 acc	 label
12.378	85.470	a
95.932	78.500	b


==> figures/data/rq-emb-mu-acc.tex <==
mu	 acc	 label
5.654728889465332	74.82	 a
5.4922051429748535	74.6	 a
5.0364227294921875	75.32	 a
4.7639689445495605	74.98	 a
5.060163497924805	74.78	 a
5.37714147567749	74.86	 a
6.936205863952637	74.62	 a
6.986508369445801	74.7	 a
5.273040771484375	74.58	 a
5.693841457366943	74.34	 a
5.629586219787598	73.68	 a


==> figures/data/rq-rep-mu-acc.tex <==
mu	 acc	 label
9.165138244628906	79.82	 b
12.534116744995117	79.3	 b
9.089764595031738	79.22	 b
9.501947402954102	79.12	 b
9.396153450012207	78.92	 b
11.29098892211914	78.9	 b
11.85473346710205	78.76	 b
10.10315990447998	78.72	 b
11.817598342895508	78.68	 b
10.040695190429688	78.88	 b
12.382781982421875	78.82	 b


==> figures/data/vr-emb-mu-acc.tex <==
mu	 acc	 label
5.646787643432617	77.8	 a
5.329698085784912	77.86	 a
4.996143341064453	77.9	 a
6.334786415100098	77.62	 a
5.841973781585693	77.54	 a
5.650638580322266	77.68	 a
5.547822952270508	77.52	 a
5.4303765296936035	78.22	 a
6.062966346740723	77.64	 a
6.514716625213623	77.32	 a


==> figures/data/vr-rep-mu-acc.tex <==
mu	 acc	 label
8.322786331176758	78.66	 b
6.995871067047119	79.24	 b
6.759679794311523	79.32	 b
7.192229747772217	79.36	 b
9.646467208862305	78.58	 b
10.620475769042969	78.22	 b
7.432973861694336	78.54	 b
9.233529090881348	79.14	 b
7.411192893981934	78.82	 b
7.332726001739502	79.02	 b

